User-Centric Gender Rewriting

In this paper, we define the task of gender rewriting in contexts involving two users (I and/or You) - first and second grammatical persons with independent grammatical gender preferences. We focus on Arabic, a gender-marking morphologically rich language. We develop a multi-step system that combines the positive aspects of both rule-based and neural rewriting models. Our results successfully demonstrate the viability of this approach on a recently created corpus for Arabic gender rewriting, achieving 88.42 M2 F0.5 on a blind test set. Our proposed system improves over previous work on the first-person-only version of this task, by 3.05 absolute increase in M2 F0.5. We demonstrate a use case of our gender rewriting system by using it to post-edit the output of a commercial MT system to provide personalized outputs based on the users' grammatical gender preferences. We make our code, data, and models publicly available.

==> results_table_MT.tex <==
\tabcolsep=3pt
\begin{table*}[ht!]
        \centering
        \begin{tabular}{|lllllllll|c|c|c|c|}
            \cline{1-13}
            
            \multicolumn{9}{|l|}{\textbf{Target}} & \textbf{1M/2M}  & \textbf{1F/2M} & \textbf{1M/2F} & \textbf{1F/2F} \\\hline\hline
            \multicolumn{9}{|l|}{\textbf {Google Translate}} &  13.8 & 13.3 & 11.7 & 11.3 \\\hline\hline
            
            \multicolumn{1}{|l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}}&  \textbf{13.9} & \textbf{13.8} & \textbf{13.5} & 13.4 \\\hline\hline
            
            \multicolumn{1}{|l}{\textbf{GID\textsubscript{Aug}}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR\textsubscript{Aug}}} & + & \multicolumn{1}{l|}{\textbf{Selection}}&  13.8 & \textbf{13.8} & \textbf{13.5} & \textbf{13.5} \\\hline
            
        \end{tabular}
        \caption{BLEU results on the post-edited Google Translate output of the {\dev} set of {\APGC} v2.0.}
        \label{tab:MT_dev_results}
    \end{table*}



\tabcolsep=3pt
\begin{table*}[ht!]
        \centering
        \begin{tabular}{|lllllllll|c|c|c|c|}
            \cline{1-13}
            
            \multicolumn{9}{|l|}{\textbf{Target}} & \textbf{1M/2M}  & \textbf{1F/2M} & \textbf{1M/2F} & \textbf{1F/2F} \\\hline\hline
            \multicolumn{9}{|l|}{\textbf {Google Translate}} &  13.6 & 13.2 & 11.4 & 11.0 \\\hline\hline
            
           \multicolumn{1}{|l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}}& \textbf{13.7} & 13.6 & \textbf{13.4} & \textbf{13.3} \\\hline\hline
            
            
            \multicolumn{1}{|l}{\textbf{GID\textsubscript{Aug}}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR\textsubscript{Aug}}} & + & \multicolumn{1}{l|}{\textbf{Selection}}&  \textbf{13.7} & \textbf{13.7} & \textbf{13.4}	& \textbf{13.3} \\\hline
            
        \end{tabular}
        \caption{BLEU results on the post-edited Google Translate output of the {\test} set of {\APGC} v2.0.}
        \label{tab:MT_test_results}
    \end{table*}


==> results_table_dev.tex <==
\tabcolsep=3.6pt
\begin{table*}[ht!]
        \centering
        \begin{tabular}{|llllllllll|c|c|c|c|}
            \cline{11-14}

            \multicolumn{10}{l|}{} & \textbf{P}  & \textbf{R} & \textbf{F\textsubscript{0.5}} & \textbf{BLEU} \\\cline{1-14}
            \multicolumn{1}{|l}{(a)} & \multicolumn{9}{l|}{\textbf{Do Nothing}} & 100.0 & 0.0 & 0.0 & 89.4 \\\cline{1-14}
             \multicolumn{1}{|l}{(b)} &\multicolumn{1}{l}{\textbf{Joint}} & + & \multicolumn{7}{l|}{\textbf{Morph}} & 64.06 &	69.56 & 65.09 & 93.3 \\\hline\hline
            
            \multicolumn{1}{|l}{(c)} &\multicolumn{1}{l}{\textbf{Joint}} & + & \multicolumn{7}{l|}{\textbf{Side Constraints}} &  79.19 & 78.91 & 79.14 & 96.0 \\\cline{1-14}
            
            \multicolumn{1}{|l}{(d)} &\multicolumn{1}{l}{\textbf{Joint}} & + & \multicolumn{1}{l}{\textbf{Morph}} & + & \multicolumn{5}{l|}{\textbf{Side Constraints}} &  80.05 & 79.91 & 80.02 & 96.3 \\\hline\hline
            
            \multicolumn{1}{|l}{(e)} &\multicolumn{1}{l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & + & \multicolumn{5}{l|}{\textbf{Selection}}  &  88.22 & 70.89 & 84.11 & 96.5 \\\cline{1-14}
            
            \multicolumn{1}{|l}{(f)} &\multicolumn{1}{l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{MorphR}} & + & \multicolumn{5}{l|}{\textbf{Selection}} & 84.16 & 76.01 & 	82.39 & 97.0  \\\cline{1-14}
            
            \multicolumn{1}{|l}{(g)} &\multicolumn{1}{l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{5}{l|}{\textbf{Selection}}& 81.87 & 67.46 & 78.52 & 96.0 \\\hline\hline
            
            \multicolumn{1}{|l}{(h)} &\multicolumn{1}{l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & + & \multicolumn{3}{l|}{\textbf{Selection}} &
            \textbf{87.95} & 86.49 & 87.65 & 98.0 \\\cline{1-14}
            
            \multicolumn{1}{|l}{(i)} & \multicolumn{1}{l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}} & 87.92 & \textbf{87.57} & \textbf{87.85} & \textbf{98.1}\\\cline{1-14}

            
        \end{tabular}
        \caption{Results of a number of systems on the {\dev} set of {\APGC} v2.0.}
        \label{tab:dev_results}
    \end{table*}


\tabcolsep=3pt
\begin{table*}[ht!]
        \centering
        \begin{tabular}{|llllllllll|c|c|c|c|}
            \cline{11-14}
            
            
            \multicolumn{10}{l|}{} & \textbf{P}  & \textbf{R} & \textbf{F\textsubscript{0.5}} & \textbf{BLEU} \\\cline{1-14}
            
            
            
            \multicolumn{1}{|l}{(a)} & \multicolumn{1}{l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR\textsubscript{Aug}}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}} & 87.78 & \bf 87.59 & 87.74 & \bf 98.1 \\\cline{1-14}
            
            \multicolumn{1}{|l}{(b)} &\multicolumn{1}{l}{\textbf{GID\textsubscript{Aug}}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}} & 88.28 & 	87.20 & 88.06 & \bf 98.1 \\\cline{1-14}
            
           \multicolumn{1}{|l}{(c)} & \multicolumn{1}{l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR\textsubscript{Aug}}} & + & \multicolumn{1}{l|}{\textbf{Selection}}& 88.03 & 87.55 & 87.93 & \bf 98.1 \\\cline{1-14}
            
            \multicolumn{1}{|l}{(d)} & \multicolumn{1}{l}{\textbf{GID\textsubscript{Aug}}} & + & \multicolumn{1}{l}{\textbf{CorpusR\textsubscript{Aug}}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}}& 88.14 & 87.24 & 87.96 & \bf 98.1 \\\cline{1-14}
            
            \multicolumn{1}{|l}{(e)} & \multicolumn{1}{l}{\textbf{GID\textsubscript{Aug}}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR\textsubscript{Aug}}} & + & \multicolumn{1}{l|}{\textbf{Selection}}& \bf 88.37 & 87.17 & \bf 88.13 & \bf 98.1 \\\cline{1-14}

            \multicolumn{1}{|l}{(f)} & \multicolumn{1}{l}{\textbf{GID\textsubscript{Aug}}} & + & \multicolumn{1}{l}{\textbf{CorpusR\textsubscript{Aug}}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR\textsubscript{Aug}}} & + & \multicolumn{1}{l|}{\textbf{Selection}} & 88.18 &	87.24 & 87.99 & \bf 98.1 \\\cline{1-14}
            
        \end{tabular}
        \caption{Data augmentation results on variants of the best system on the {\dev} set of {\APGC} v2.0. $\alpha$ indicates that the component of the system is trained on the augmented data.}
        \label{tab:dev_results_aug}
    \end{table*}


==> results_table_test_new.tex <==
\tabcolsep=3pt

\begin{table*}[ht!]
        \centering
        \begin{tabular}{|lllllllll|c|c|c|c|}
            \cline{10-13}
            \multicolumn{9}{l|}{} & \textbf{P}  & \textbf{R} & \textbf{F\textsubscript{0.5}} & \textbf{BLEU} \\\cline{1-13}
            
            \multicolumn{1}{|l}{\textbf{Joint}} & + & \multicolumn{1}{l}{\textbf{Morph}} & + & \multicolumn{5}{l|}{\textbf{Side Constraints}} & 81.05 & 80.47 & 80.93  & 96.5 \\\hline\hline
            
            \multicolumn{1}{|l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}} & 88.06	& 86.76 & 87.80 & 98.0 \\\hline\hline
            
            \multicolumn{1}{|l}{\textbf{GID\textsubscript{Aug}}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
            \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR\textsubscript{Aug}}} & + & \multicolumn{1}{l|}{\textbf{Selection}} & \bf 88.41 & \bf 86.80 & \bf 88.08 & \bf 98.0 \\\hline
            
\multicolumn{13}{c}{\vspace{0.5cm}}\\

        \cline{10-13}
        
        \multicolumn{9}{l|}{} & \textbf{P}  & \textbf{R} & \textbf{F\textsubscript{0.5}} & \textbf{BLEU} \\\cline{1-13}
        
        \multicolumn{9}{|l|}{\textbf{\newcite{habash-etal-2019-automatic}}}&  77.7 & 52.0 & 70.8 & 98.3 \\\hline\hline
        \multicolumn{9}{|l|}{\textbf{\newcite{alhafni-etal-2020-gender}}}&  \textbf{79.0} & 60.3 & 74.4 & 98.5 \\\hline\hline
        \multicolumn{1}{|l}{\textbf{GID}} & + & \multicolumn{1}{l}{\textbf{CorpusR}} & >> &
        \multicolumn{1}{l}{\textbf{MorphR}} & >> & \multicolumn{1}{l}{\textbf{NeuralR}} & + & \multicolumn{1}{l|}{\textbf{Selection}} & 76.96 & \textbf{74.31} & \textbf{76.42} & \textbf{98.9} \\\hline
        
        \end{tabular}
        \caption{Gender Rewriting Results on the {\test} set of {\APGC} v2.0.}
        \label{tab:test_results}
\end{table*}

